A Differential Testing Approach for Evaluating Abstract Syntax Tree Mapping Algorithms

Abstract syntax tree (AST) mapping algorithms are widely used to analyze changes in source code. Despite the foundational role of AST mapping algorithms, little effort has been made to evaluate the accuracy of AST mapping algorithms, i.e., the extent to which an algorihtm captures the evolution of code. We observe that a program element often has only one best-mapped program element. Based on this observation, we propose a hierarchical approach to automatically compare the similarity of mapped statements and tokens by different algorithms. By performing the comparison, we determine if each of the compared algorithms generates inaccurate mappings for a statement or its tokens. We invite 12 external experts to determine if three commonly used AST mapping algorithms generate accurate mappings for a statement and its tokens for 200 statements. Based on the experts' feedback,we observe that our approach achieves a precision of 0.98--1.00 and a recall of 0.65--0.75. Furthermore, we conduct a large-scale study with a dataset of ten Java projects, containing a total of 263,165 file revisions. Our approach determines that GumTree, MTDiff and IJM generate inaccurate mappings for 20%--29%, 25%--36% and 21%--30% of the file revisions, respectively. Our experimental results show that state-of-art AST mapping agorithms still need improvements.

==> manual.tex <==
%In this section, we describe overview and details of our approach.
%Notice that our approach is general, although we explain it for Java.

From our manual analysis, we have the following findings.

\begin{itemize}

\item The Kappa value for the two annotators' determination results is 0.81.
Hence, the determination results of the two annotators have an excellent agreement.

\item Among the 178 statements for comparing GT and MTD, 71 and 129 statements involve inaccurate mappings as generated by GT and MTD, respectively.

\item Among the 191 statements for comparing GT and IJM, 114 and 91 statements involve inaccurate mappings as generated by GT and IJM, respectively.

\item Among the 206 statements for comparing MTD and IJM, 113 and 117 statements involve inaccurate mappings as generated by MTD and IJM, respectively.

\item For each statement with inconsistent mappings for comparing two algorithms, at least one algorithm is determined to generate inaccurate mappings. Hence, statements with inconsistent mappings can expose the inaccurate mappings as generated by the algorithms.

\item There exist cases where two algorithms consistently produce an inaccurate mapping of a statement or a token.
\end{itemize}

\input{tables/measures}

In total, we find 186 ($72+114$), 247 ($130+117$), 208 ($91 + 117$) statements with inaccurate mappings for GT, MTD and IJM, respectively.
Based on our observation, we design two similarity measures for comparing two statements and four similarity measures for comparing two tokens.
Table~\ref{tab:measure} presents the six measures.
Notice that we define two tokens with the same value as \emph{identical tokens}.
Besides, based on our analysis, we propose the usage of the measures when comparing the generated mappings by different algorithms.
In the remaining part of this section, we first elaborate the six measures and introduce our categorization results for the statements with inaccurate mappings.
Then we describe the usage of the measures.
%Table~\ref{tab:measure} presents the measures and the number of statements categorized along the measures.
%The measures can identify 157 (84\%), 208 (84\%) and 178 (86\%) of the statements with inaccurate mappings for GT, MTD and IJM.
%The other statements with inaccurate mappings are categorized into the \textbf{Other} category.
%For these statements, we find that determining accuracy of the mappings of statements and tokens requires more comprehension of the changes.
%and how to use the measures to automatically compare the generated mappings between different algorithms

%And we define tokens of a pair of mapped statements except mapped identical tokens as \emph{changed tokens} of the two statements.

\subsection{Similarity Measures}

The six similarity measures are elaborated below.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.5\textwidth]{pictures/measure1.pdf}\\
  \caption{Illustrative examples of inaccurately mapped statements that can be identified using our measures.}\label{fig:measure1}
\end{figure}

\textbf{NIT} is defined as the number of mapped identical tokens between a pair of mapped statements.
Two mapped statements with a larger NIT are more similar and an NIT of 0 indicates the two statements are highly dissimilar.
If two statements are mapped with an NIT of 0, we determine the mapping as inaccurate.
Otherwise, for a pair of mapped statements, we check if mapping one of the statements to another statement can achieve a larger NIT.
%When two algorithms map a statement to different statements, we observe that the mapped statements that have more identical tokens are more similar.
For instance, in Fig.~\ref{fig:measure1}(a), MTD inaccurately maps the statements at lines 1 and 2 and the NIT is 0.
In Fig.~\ref{fig:measure1}(b), GT maps the statements at lines 1 and 2 with an NIT of five.
IJM maps the statements at lines 1 and 3 with an NIT of four.
We determine that GT is more accurate than IJM in mapping the statement at line 1.

%\textbf{NCT} is defined as the number of changed tokens between a pair of mapped statements.
%We observe that the mapped statements with less NCT are more similar.
%For a pair of mapped statements, we check if mapping one of the statements to another statement can achieve the same NIT and a less NCT.
%When two algorithms map a statement to different statements, we compare NCT between the two pairs of mapped statements if they have the same NIT.
%For instance, in Fig.~\ref{fig:measure1}(c), GT maps the statements at lines 1 and 2 with an NCT of 2, while IJM maps the statement at line 1 itself with an NCT of 0.
%Using the measure, we determine that IJM is more accurate than GT in mapping the statement at line 1.

\textbf{PM} characterizes whether the parent nodes of a pair of mapped statements are also mapped.
%When two algorithms map a statement to different statements, we compare PM between the two pairs of mapped statements if they have the same NIT and NCT.
We observe that the mapped statements with mapped parent nodes are more similar.
For a pair of mapped statements, we check if mapping one of the statements to another statement with mapped parent nodes can achieve the same NIT.
For instance, in Fig.~\ref{fig:measure1}(d), IJM maps the statements at lines 1 and 2 with mapped parent nodes, while GT maps the statements at lines 1 and 3 with parent nodes not mapped.
We determine that IJM is more accurate than GT in mapping the statement at line 1.
Furthermore, we notice a special type of statements, i.e., blocks.
A block is a group of statements between balanced braces (i.e., ``\{'' and ``\}'').
We observe that a block should be mapped along with its parent nodes, e.g., the ``\{'' following the method \texttt{testFilterSet} in Fig.~\ref{fig:measure1}(d) should be mapped along with the method declaration.
Thus, mapped blocks with unmapped parent nodes are determined to be inaccurate.



\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=0.5\textwidth]{pictures/measure2.pdf}\\
  \caption{Illustrative examples of inaccurately mapped tokens that can be identified using our measures.}\label{fig:measure2}
\end{figure}

\textbf{TYPE} characterizes whether mapped tokens have the same type.
For a token whose directly relevant node is not a name node, we define the type of the token as the label of its directly relevant node.
For tokens whose directly relevant node is a name node, we define four types: variable name, type name, method name and declaration name.
Following Frick et al.~\cite{frick2018generating}, we consider that mapping tokens with different types are inaccurate.
For instance, in Fig.~\ref{fig:measure2}(a), GT maps a variable name \texttt{value} to a method name \texttt{bytevalue}, we determine the mapping as inaccurate.
For an algorithm that maps two tokens of different types, we determine the mapping as inaccurate.

\textbf{STMT} characterizes whether mapped tokens belong to a pair of mapped statements.
%We use this measure when two algorithms map a statement $s$ to the same statement and map a token of $s$ to different tokens with the same type.
Two tokens from mapped statements are more likely to be mapped.
We observe that mapping tokens from mapped statements is better than (1) not mapping the tokens and (2) mapping tokens from unmapped statements.
For instance, in Fig.~\ref{fig:measure2}(b), the two \texttt{value} tokens are both variable names and they belong to a pair of mapped statements.
GT maps the two tokens, while IJM does not map them.
We determine that GT is more accurate than IJM in mapping the two tokens.
In Fig.~\ref{fig:measure2}(c), GT maps the two \texttt{HashMap} tokens in unmapped statements, while IJM maps the \texttt{HashMap} to the \texttt{Map}, and the two tokens belong to mapped statements.
Using the STMT measure, we determine that IJM is more accurate in mapping the \texttt{HashMap} at line 1 than GT.


\textbf{VAL} characterizes whether mapped tokens have the same string value.
%We use this measure when two algorithms map a statement $s$ to the same statement and map a token of $s$ to different tokens that satisfy the conditions of TYPE and STMT.
%We consider that the similarity of two tokens with the same value is larger than that of two tokens with different values.
Two identical tokens in a pair of mapped statements are more likely to be mapped.
We consider that mapping such two tokens is better than mapping one of the tokens to another token with different values between the two statements.
For instance, in Fig.~\ref{fig:measure2}(d), GT maps \texttt{getBytes} to \texttt{writeBytes}, while IJM maps the two \texttt{getBytes} tokens.
Using the VAL measure, we determine that IJM is more accurate in mapping the \texttt{getBytes} tokens than GT.


\textbf{LLCS} is defined as the length of the longest common subsequence (LCS)~\cite{hirschberg1977algorithms} calculated using the mapped tokens between mapped statements.
%We use this measure when two algorithms map a statement $s$ to the same statement and map a token of $s$ to different tokens that satisfy the conditions of TYPE, STMT and VAL.
We observe that orders of tokens are not frequently changed in a statement.
We use LLCS to quantify the number of tokens that are sequentially mapped between the mapped statements.
For instance, in Fig.~\ref{fig:measure2}(e), GT changes the orders of the two \texttt{Filterable} tokens in the statement at line 1.
As a result, at most three tokens are sequentially mapped between the statements, i.e., \texttt{Filterable}, \texttt{=} and \texttt{runner}.
The LLCS for the mapped tokens is calculated as three.
IJM sequentially maps the five tokens between the two statements.
The LLCS for the mapped tokens is calculated as five.
Using the LLCS measure, we determine that IJM is more accurate in mapping the \texttt{Filterable} tokens than GT.

Table~\ref{tab:measure} shows the number of statements categorized along the measures.
The measures can identify 157 (84\%), 208 (84\%) and 178 (86\%) of the statements with inaccurate mappings for GT, MTD and IJM.
The other statements with inaccurate mappings are categorized into the \textbf{Other} category.
For these statements, we find that determining accuracy of the mappings of statements and tokens requires more comprehension of the changes.

\subsection{Usage of the Similarity Measures}

We compare the generated mappings by two algorithms by taking the following steps.

\noindent\textbf{Step 1.}
If an algorithm maps two non-block statements with an NIT of 0, we determine the mapping as inaccurate.
If an algorithm maps two blocks with unmapped parent nodes, we determine the mapping as inaccurate.
If an algorithm maps two tokens with different types, we determine the mapping as inaccurate.

\noindent\textbf{Step 2.}
When the two algorithms map a statement to different statements, mapping statements with a larger NIT is considered to be better.
If the two pairs of statements have the same NIT, mapping statements with mapped parent nodes is considered to be better than mapping statements with unmapped parent nodes.

\noindent\textbf{Step 3.}
When the two algorithms consistently map a statement $s$, we assume that the two algorithms accurately map $s$.
From $s$, we retrieve all the tokens that are inconsistently mapped by the two algorithms.
For a token that is inconsistently mapped by the two algorithms, we first use the STMT measure to compare the generated mappings for the token by the two algorithms.
If both algorithms map tokens from the mapped statements, mapping identical tokens is considered to be better than mapping tokens with different values.
If both algorithms map identical tokens from the mapped statements, the mapped tokens with larger LLCS are considered to be better.


%When two algorithms map a statement to different statements, we sequentially use the NIT and PM measures to compare the two pairs of mapped statements.
%When an algorithm maps two tokens with different types, we use the TYPE measure and determine the mapping that is inaccurate.
%When two algorithms consistently map a statement, we assume that the two algorithms accurately map the statement.
%We sequentially use the STMT, VAL and LLCS measures to compare mappings of tokens in the statement as generated by the two algorithms.


%We categorize the statements with inaccurate mappings that cannot be detected using our measures into the \textbf{Other} category.
%Determining the inaccurate mappings in these statements requires more syntactic information from the code (e.g., data flow and control flow).
%For instance, we observe cases where an algorithm may map two tokens from unmapped statements, while another algorithm do not map the tokens.
%We cannot determine whether the two tokens should be mapped without understanding the changes.
%Furthermore, we also find cases where two algorithms consistently map a statement or a token and the mapping is determined to be inaccurate.


==> settings.tex <==

In this section, we first introduce the studied AST mapping algorithms and analyzed projects.
Then, we describe the steps to prepare the analyzed data, i.e., statements with inconsistent mappings for comparing different algorithms.
Next, we elaborate the settings of our manual analysis.
%Based on the analysis, we derive measures to quantify the similarity between two statements or two tokens.
We finally describe our approach to compare the similarity of mapped statements and tokens by different algorithms and determine the accuracy of the algorithms.
Notice that our approach is general.
We implement it for Java programs but we can modify it to support other programs as long as we can generate ASTs from them.

%Then, we further elaborate data preparation, manual analysis and the comparison approach.
%In our study, we first calculate statements with inconsistent mappings by comparing different algorithms for further analyses.
%Then, we manually analyze a sample of statements with inconsistent mappings.
%Based on the analysis, we derive measures to quantify the similarity between two statements or two tokens.
%Next, we implement an automatic approach to compare the similarity of mapped statements and tokens by different algorithms.
%Finally, we use our approach to automatically analyze the file revisions of the studied projects.



In this paper, we aim to answer three research questions:

\noindent\emph{RQ1: Can we effectively find the inaccurate mappings as generated by the studied algorithms?}

\noindent\emph{RQ2: How effective is our approach when comparing an algorithm with multiple algorithms than when comparing it with \textcolor{red}{another} algorithm?}

\noindent\emph{RQ3: Do state-of-the-art AST mapping algorithms generate many inaccurate mappings?}


\subsection{Studied Algorithms}
In this study, we analyze three state-of-the-art AST mapping algorithms, namely GumTree~\cite{falleri2014fine}, MTDiff~\cite{dotzler2016move} and IJM~\cite{frick2018generating}.
We briefly introduce the three algorithms below.

\textbf{GumTree (GT)} is proposed by Falleri et al~\cite{falleri2014fine}.
Given two ASTs, GT matches nodes between the ASTs in two phases:
In the first phase, GT applies a greedy top-down algorithm to search and map identical subtrees.
In the second phase, GT applies a bottom-up algorithm to map a pair of nodes between the two ASTs if they share a significant number of mapped descendants.
Then, GT tries to map previously unmapped descendants of those nodes.
%If the two nodes are mapped, GT further applies the RTED algorithm (a tree-based mapping algorithm that does not consider moved nodes)~\cite{pawlik2011rted} to map descendants of the two nodes.

\textbf{MTDiff (MTD)} is proposed by Dotzler et al.~\cite{dotzler2016move}.
MTD is based on the ChangeDistiller algorithm~\cite{fluri2007change}.
First, MTD applies the identical subtree optimization to reduce the mapping problem by removing unchanged subtrees from the ASTs.
Then, MTD maps nodes using the ChangeDistiller algorithm.
Another four optimizations are finally applied to find additional mappings of nodes.

\textbf{IJM} is proposed by Frick et al.~\cite{frick2018generating}.
IJM is the abbreviation of Iterative Java Matcher.
IJM is an AST mapping algorithm specialized for Java.
In comparison to GT, IJM works on a reduced AST, in which many name nodes are pruned and the value of each pruned node is merged to its parent node.
Then, IJM splits the AST into parts along each declaration.
Finally, it maps AST nodes from the corresponding parts between the two ASTs using an adaptation of the GT algorithm.
The adaptation adds name-awareness to GT, which considers similarity of values when mapping two nodes.

%ChangeDistiller is an AST mapping algorithm.
%It works on ASTs that only encode statements.
%Given two ASTs, ChangeDistiller first maps leaf nodes according to string similarity, and then, it iteratively maps non-leaf nodes that have a significant number of mapped descendants.
%Dotzler et al. adapted the ChangeDistiller algorithm on GT's ASTs, in which fine-grained code tokens are encoded as nodes.


%Then, IJM splits ASTs into several parts including: import declarations, type declarations, method declarations, enumeration declarations and field declarations.
%All of the name nodes in GumTree's ASTs have the same label (i.e., \texttt{SimpleName}).
%As described in Section~\ref{preliminary}, AST mapping algorithms map the nodes with the same label.
%Frick et al. noted that mapping a pair of name nodes should consider their parent nodes, e.g., a method name should not be mapped to a variable name~\cite{frick2018generating}.
%Hence, they pruned name nodes to avoid mapping name nodes everywhere.

In this study, we apply the implementations of the three algorithms that are provided on GitHub~\cite{gumtreeGitHub, mtdiffGitHub, ijmGitHub}.
%In addition, we exclude ChangeDistiller from our analysis since ChangeDistiller works on coarse-grained AST nodes and we cannot calculate mappings of tokens based on mappings of such AST nodes.
%Furthermore, AST mapping algorithms that work on fine-grained AST nodes are preferred by researchers since more detailed edit actions can be derived from the generated mappings~\cite{frick2018generating}.
%Algorithms using fine-grained AST nodes (e.g., GumTree) are more likely to be used in future studies.



%We have two goals in answering this question.
%First, we investigate whether the inconsistent mappings generated by two algorithms can expose the inaccurate mappings as generated by both algorithms.

\subsection{Studied Projects}
We analyze ten open-source Java projects in this study.
Table~\ref{tab:projects} presents statistics of the studied projects.
These projects were analyzed by prior studies~\cite{huang2018cldiff, frick2018generating}.
We collect the commits of the projects from the creation date of the projects to January 2019.

\begin{table}
  \centering
  \scriptsize
  \caption{Statistics of the studied projects.}
    \begin{tabular}{|l|r|r|}
    \hline
    \textbf{Projects} & \multicolumn{1}{l|}{\textbf{\#Commit}} & \multicolumn{1}{l|}{\textbf{\#Revision}} \\
    \hline
    ActiveMQ &                8,059  &                24,813  \\
    Commons IO &                1,067  &                  2,727  \\
    Commons Lang &                3,031  &                  6,917  \\
    Commons Math &                4,257  &                18,133  \\
    Junit4 &                1,241  &                  3,802  \\
    Hibernate ORM &              10,170  &                51,711  \\
    Hibernate Search &                5,369  &                27,002  \\
    Spring Framework &              14,754  &                68,413  \\
    Spring Roo &                4,274  &                19,894  \\
    Netty &              11,135  &                39,753  \\
    \hline
    \textbf{Total} &              63,357  &              263,165  \\
    \hline
    \end{tabular}%
  \label{tab:projects}%
\end{table}%


\subsection{Data Preparation}

% overview of our framework


%\begin{figure}
%  \centering
%  % Requires \usepackage{graphicx}
%  \includegraphics[width=0.5\textwidth]{pictures/framework.pdf}\\
%  \caption{Data preparation steps.}\label{fig:overview}
%\end{figure}

%Fig.~\ref{fig:overview} presents the overview of our approach.
%Given two AST mapping algorithms and a file revision, we analyze the generated mappings by the algorithms in two phases.
%In the first phase, we calculate statements with inconsistent mappings.
%In the second phase, for each statement with inconsistent mappings, we determine the accuracy of each algorithm in mapping the statement and its tokens.

%We face two challenges in calculating the inconsistent mappings by comparing two algorithms.
%First, different algorithms use ASTs with different sets of nodes (including leaf nodes) to represent the same file.
%For instance, in comparison to IJM's AST, GumTree's AST encodes more tokens as nodes (e.g., the first \texttt{HashMap} of line 1 in Fig.~\ref{fig:mapping-example}(a)).
%Finding the corresponding nodes from the ASTs used by different algorithms is a big challenge.
%Second, the granularity of AST nodes ranges from statements to a single token (e.g., a variable name).
%It is too complex to analyze the mappings for AST nodes of all granularity levels.
%We observe that different algorithms commonly encode statements as AST nodes.
%Furthermore, tokens of a statement are not sensitive towards to nodes composing the statement in an AST.
%In this paper, a token is defined as a sequence of characters representing a program element such that none of its subsequence represents a program element.
%Thus, we take two measures to tackle the challenges: (1) we treat each statement as an analysis unit; and (2) we project the mappings of AST nodes in each statement as mappings of tokens as shown in Fig.~\ref{fig:token-mappings}.
% Instead of analyzing the mappings of statements and tokens one by one, w

We calculate the inconsistent mappings by comparing each pair of studied algorithms for further analyses.
The granularity of AST nodes ranges from a statement to a single literal.
It is too complex to analyze mappings of AST nodes of all granularity levels.
Furthermore, finding the corresponding nodes from the used ASTs by different algorithms is a big challenge.
Because different algorithms may use ASTs with different sets of nodes (including leaf nodes) to represent the same file, as shown in Fig.~\ref{fig:mapping-example} and Fig.~\ref{fig:mappings-ijm}.
We observe that different algorithms commonly encode statements as AST nodes.
Additionally, tokens of a file are not impacted by the composing nodes of an AST.
To solve the above issues, we refine mappings of AST nodes into mappings of statements and tokens.
Moreover, we treat each statement (including the statement itself and its tokens) as an analysis unit.


Given a file revision, we take four steps to compare two algorithms and calculate the statements with inconsistent mappings: (1) tokenization, (2) grouping mappings along statements, (3) creating mappings of statements and tokens, and (4) calculating statements with inconsistent mappings.
We describe the steps as follows.

\noindent\underline{\emph{(1) Tokenization.}}
In this step, we tokenize the file before and after a revision.
Instead of using punctuation and spaces, we use the parsed AST of the source file to tokenize the file.
For example, a string literal containing punctuation and spaces is considered as a single token.

For a Java file, we first use the Eclipse JDT parser to generate a standard JDT AST.
Then, we extract the tokens from value of each AST node.
Notice that we ignore AST nodes representing comments and Javadocs.
Because comments and Javadocs are typically not treated as code~\cite{huang2018cldiff}.
As a result, we retrieve two token lists for a file before and after a revision, respectively.
The token lists are not impacted by the used AST by each algorithm

%By tokenizing a file, we retrieve a universal token list that is not impacted by the ASTs used by different algorithms.


%As a result, we calculate two lists of tokens for the file before and after the revision, respectively.

%We use the characters ``('', ``)'', ``.'', ``:'', ``?'', ``['', ``]'', ``\{'' and ``\}'' as punctuation.
%The characters ``\texttt{<}'' and ``\texttt{>}'' are also used as punctuation when they are not used as operators of infix expressions (e.g., \texttt{a >= b}).
%Besides, we consider the syntactic structure of code when tokenizing a source file.
%For example, a string literal containing punctuation and spaces is considered as a single token.
%As another example, the expression \texttt{a+b} that contains no punctuation and space can be split as ``a'', ``+'' and ``b'' by considering the syntactic structure of code.
%As described earlier, GT's AST encodes more tokens as nodes than IJM's AST.
%Hence, we use GT's AST to represent a Java file.
%Each node in the AST represents a program element.
%We record the start and end character positions of the corresponding program elements for all the AST nodes.

%To tokenize a Java file, we first prune comments and Javadocs away from the file using regular expressions.
%Because comments and Javadocs are typically not treated as code~\cite{huang2018cldiff}.
%Then, we extract all the literals from the file by using the AST representing the file.
%The string value of these literals are stored as tokens, and we prune the literals away from the file.
%After that, we leverage punctuation and spaces to split the remaining content of the file as many sequences of characters.
%Some sequences may be further split by considering the syntactic structure of code, e.g., \texttt{a+b}.
%Finally, each sequence of characters is further split at each start and end character positions of the program elements that we record.


\noindent\underline{\emph{(2) Grouping mappings along statements.}}
In this step, we separately group mappings of AST nodes along statements for the two algorithms that are being compared.
In an AST, a statement (e.g., a method declaration) can have descendant statements.
For each statement in the source and target ASTs that are being analyzed by an algorithm, we first group the nodes that belong to the statement but do not belong to its descendant statements.
For instance, our framework groups $n_1$, $n_2$, and $n_3$ in Fig.~\ref{fig:mapping-example}(b) for the type declaration \texttt{PublishedAddressPolicy}.
Then, we find the generated mappings by the algorithm for the grouped nodes.
These mappings are grouped for the statement.



\noindent\underline{\emph{(3) Creating mappings of statements and tokens.}}
In this step, we separately calculate mappings of statements and tokens for the two algorithms.
Among the grouped mappings for each statement, we can directly find the mapping for the statement.
For instance, in Fig.~\ref{fig:mapping-example}(b), $n_1$ represents the type declaration \texttt{PublishedAddressPolicy} and the mapping of $n_1$ is considered as the mapping of the declaration.

For a token, we refer to an AST node whose corresponding program element contains the token as a \emph{relevant node} of the token.
Among the relevant nodes of a token, we refer to the node of the lowest level as the \emph{directly relevant node} of the token.
In return, we refer to the token as a \emph{directly relevant token} of the node.
We take the first \texttt{HashMap} of line 1 in Fig.~\ref{fig:mapping-example}(a) as an example.
In the used AST by GT shown in Fig.~\ref{fig:mapping-example}(b), $n_1$, $n_4$, $n_6$, $n_7$ and $n_8$ are relevant nodes of the token.
And the directly relevant node for the token is $n_8$.
In the used AST by IJM shown in Fig.~\ref{fig:mappings-ijm}(a), $n_1$, $n_3$ and $n_5$ are relevant nodes of the token.
And the directly relevant node for the token is $n_5$.

An AST node can have several directly relevant tokens.
For instance, the node $n_5$ in Fig.~\ref{fig:mappings-ijm}(a) has three directly relevant tokens including a \texttt{HashMap} and two \texttt{Integer} tokens.
Such tokens compose the value of $n_5$.
Another example is $n_1$ in Fig.~\ref{fig:mappings-ijm}, which has two directly relevant tokens including the \texttt{class} and \texttt{PublishedAddressPolicy} tokens in Fig.~\ref{fig:mapping-example}(a).
The \texttt{PublishedAddressPolicy} token is the value of the node, while the \texttt{class} does not belong to its value.

We observe that a token's mapping is determined by the mapping of its directly relevant node.
We also take the first \texttt{HashMap} of line 1 in Fig.~\ref{fig:mapping-example}(a) as an example.
In Fig.~\ref{fig:mapping-example}, GT maps $n_8$ to $n_{61}$---indicating that the token is mapped to the \texttt{HashMap} of line 3 in Fig.~\ref{fig:mapping-example}(a).
And in Fig.~\ref{fig:mappings-ijm}, IJM maps $n_5$ to $n_{13}$---indicating that the token can only be mapped to a directly relevant token of $n_{13}$.

For each node of the source and target ASTs, we calculate all the directly relevant tokens and list the tokens according to their character positions.
Then, for each pair of mapped nodes, we map tokens from the lists of directly relevant tokens of the nodes.
If both lists have only one token, we directly map two tokens.
Otherwise, we separately map the tokens composing the value of the nodes and other tokens, since tokens composing the value of a node can only be mapped to those composing the value of another node.
For the tokens composing the values of the two nodes, we first sequentially map identical tokens between the two lists and then map the tokens (including the first and last tokens) that are surrounded by already mapped pairs of tokens.
Mapping program elements surrounded by already mapped pairs is a commonly used heuristic by program element mapping algorithms~\cite{kim2006program}.
After that, our framework applies the same method to map the tokens that do not belong to the value of the two nodes.

For instance, in Fig.~\ref{fig:mappings-ijm}, $n_5$ and $n_{13}$ are mapped.
The directly relevant tokens of $n_5$ include \texttt{HashMap}, \texttt{Integer} and \texttt{Integer}.
And the directly relevant tokens of $n_{13}$ include \texttt{Map}, \texttt{Integer} and \texttt{Integer}.
All of the tokens belong to the values of the two nodes.
We first sequentially map the two \texttt{Integer} between the two lists.
\texttt{HashMap} and \texttt{Map} are surrounded by already mapped tokens and they are further mapped.

As a result, we calculate mappings of tokens using the generated mappings of the AST nodes by the two algorithms.
We further group mappings of tokens along each statement based on the mappings of grouped AST nodes of the statement.

\noindent\underline{\emph{(4) Calculating statements with inconsistent mappings.}}
In this step, we compare the mappings of statements and tokens between the two algorithms being compared.
For each statement in the file before and after the revision, we first calculate whether the two algorithms inconsistently map the statement.
Then, for each token in the statement, we calculate whether the two algorithms inconsistently map the token.
Finally, we output statements with inconsistent mappings and for each statement, we group the inconsistent mappings of the statement and its tokens by comparing the two algorithms.

\subsection{Manual Analysis}

%In this phase, we determine the accuracy of each algorithm for each statement with inconsistent mappings.
%Given a statement with inconsistent mappings, we take two steps: (1) calculating similarity measures and (2) comparing similarity measures.
%We describe the steps as follows.

%\noindent\underline{\emph{(1) Calculating similarity measures.}}
%In this step, we calculate nine measures to quantify the similarity between mapped statements and tokens (five for statements and four for tokens).
%We use the similarity measures to estimate the likelihood of being mapped for two statements or tokens.
%For the statement with inconsistent mappings, we separately calculate the nine measures based on the generated mappings by the two algorithms

We perform a manual analysis of statements with inconsistent mappings.
We have two aims: (1) verifying whether statements with inconsistent mappings can expose the inaccurate mappings as generated by the algorithms;
(2) designing measures to quantify the similarity between two statements and two tokens.

We can compare three pairs of algorithms, namely GT vs. MTD, GT vs. IJM and MTD vs. IJM.
For each pair of algorithms, we sample 50 file revisions for which the two algorithms inconsistently map program elements.
For each file revision, we analyze all the statements before and after the revision that involve the inconsistent mappings.
We analyze 178, 191 and 206 statements for comparing the three pairs of algorithms, respectively.
In total, we analyze 575 statements.
For each statement, we determine the accuracy of mappings as generated by each of compared algorithm using Frick et al.'s criteria~\cite{frick2018generating}.
In total, we make 1,150 ($575 \times 2$) determinations.

The first and second author of this paper separately analyzed the statements with inconsistent mappings.
Both authors have multiple years of programming experience in Java.
We calculate Fleiss' Kappa~\cite{fleiss1971measuring} to estimate the agreement of the two annotators' determination results.
According to Fleiss' guisdelines~\cite{fleiss2013statistical}, a Kappa value of larger than 0.75 indicates an excellent agreement.
Finally, the two authors compared their determination results to uncover disagreements.
For each statement with a disagreement, the authors further discussed the accuracy of the generated mappings by the two compared algorithms.

For each file revision, we analyze all the statements with inaccurate mappings for an algorithm.
We consider if there is a similarity measure that can distinguish the accurate and inaccurate mapping of a statement or a token.
Then, we use the card sorting method to categorize the statements with inaccurate mappings for the algorithms along each similarity measure.

%Then, we design similarity measures to distinguish accurate and inaccurate mappings of statements and tokens.


\subsection{Comparison Approach}\label{approach}

%\noindent\underline{\emph{(2) Comparing Similarity Measures.}}
%In this step, for each inconsistently mapped program element $e$ (statement or token) by the two algorithms, we compare the similarity between $e$ and mapped elements by the two algorithms.
%We consider that the algorithm mapping more similar statements and tokens is more likely to be accurate.
%And the other algorithm is considered to be inaccurate.

Based on the similarity measures derived from our manual analysis, we compare the similarity of mapped statements and tokens across each pair of different algorithms.
By performing the comparison, we aim to determine the accuracy of each algorithm in the mapping of a statement or a token.


Let us denote the similarity between two program elements $e$ and $\hat{e}$ as $Sim(e, \hat{e})$.
The elements can be statements or tokens.
Suppose that two algorithms ($A_0$ and $A_1$) map a program element $e_0$ to two different elements $e_1$ and $e_2$, respectively.
We notice that the two algorithms also inconsistently map $e_1$ and $e_2$.
Suppose that $A_0$ maps an element $e_3$ to $e_2$, and $A_1$ maps an element $e_4$ to $e_1$.
In other words, $A_0$ generates two mappings $\{\langle e_0, e_1\rangle, \langle e_3, e_2\rangle\}$.
And $A_1$ generates two mappings $\{\langle e_0, e_2\rangle, \langle e_4, e_1\rangle\}$.

Suppose that $Sim(e_0, e_1)$ is larger than $Sim(e_0, e_2)$, we determine that $A_0$ is more accurate than $A_1$ in mapping $e_0$.
However, it is not enough to determine that the mapping of $e_0$ to $e_1$ is better than the generated mappings by $A_1$.
We must also check the condition: $Sim(e_0, e_1) > Sim(e_4, e_1)$, i.e., $A_0$ is also more accurate than $A_1$ in mapping $e_1$.
If this condition is also satisfied, we determine that $A_1$ inaccurately maps $e_0$ and $e_1$.
Similarly, we can also determine if the two generated mappings by $A_0$ are inaccurate.

%To determine that mapping $e_0$ and $e_1$ is better than the generated mappings by $A_1$, we must also check the condition: $Sim(e_0, e_1) < Sim(e_4, e_1)$, i.e., $A_0$ is also more accurate than $A_1$ in mapping $e_1$.
%We determine if the generated mappings by $A_1$ are inaccurate using the two conditions.
%Similarly, we determine if the
%If $Sim(e_0, e_1)$ is larger than both $Sim(e_0, e_2)$ and $Sim(e_4, e_1)$, we consider that mapping $e_0$ and $e_1$ is better than the generated mappings by $A_1$.
%We determine that the two generated mappings by $A_1$ are inaccurate.
%Otherwise, if $Sim(e_0, e_2)$ is larger than both $Sim(e_0, e_1)$ and $Sim(e_3, e_2)$, we consider that mapping $e_0$ and $e_2$ is better than the generated mappings by $A_0$.
%We determine that the two generated mappings by $A_0$ are inaccurate.


Given a pair of algorithms and a file revision, we calculate the statements with inconsistent mappings.
For each statement with inconsistent mappings, we perform the above comparison for the mappings of the statement and its tokens as generated by the two algorithms that are being compared.
Consequently, we calculate statements with inaccurate mappings for each algorithm.
For each studied algorithm, we separately compare it with the other two algorithms.
Finally, we calculate a union set of statements with inaccurate mappings for any of the algorithms that are being compared.

%For example, if $Sim(e_0, e_1)$ is less than $Sim(e_0, e_2)$, we conclude that $e_2$ is more likely to be mapped to $e_0$ than $e_1$.
%But if $Sim(e_3, e_2)$ is larger than $Sim(e_0, e_2)$, we conclude that .

%With the conflicted conclusions, we cannot determine whether


